ManyDSL: A Host for Many Languages

Domain-specific languages are becoming increasingly important. Almost every application touches multiple domains. But how to define, use, and combine multiple DSLs within the same application? The most common approach is to split the project along the domain boundaries into multiple pieces and files. Each file is then compiled separately. Alternatively, multiple languages can be embedded in a flexible host language: within the same syntax a new domain semantic is provided. In this paper we follow a less explored route of metamorphic languages. These languages are able to modify their own syntax and semantics on the fly, thus becoming a more flexible host for DSLs. Our language allows for dynamic creation of grammars and switching languages where needed. We achieve this through a novel concept of Syntax-Directed Execution. A language grammar includes semantic actions that are pieces of functional code executed immediately during parsing. By avoiding additional intermediate representation, connecting actions from different languages and domains is greatly simplified. Still, actions can generate highly specialized code though lambda encapsulation and Dynamic Staging.

==> acknowledgement.tex <==
\acks
This work is partly supported by the Federal Ministry of Education and Research (BMBF), as part of the ECOUSS project, and by the Intel Visual Computing Institute (IVCI) Saarbrücken. It is also co-funded by the European Union (EU), as part of the Dreamspace project.


==> template/tikzshapes.tex <==
\makeatletter
%\tikzset{arc style/.initial={}}
\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
% compute corner of ?flipped page?
\pgf@xc=\pgf@xb \advance\pgf@xc by-10pt % this should be a parameter
\pgf@yc=\pgf@yb \advance\pgf@yc by-10pt
% construct main path
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
}
}
\makeatother

\tikzstyle{document}=[shape=document,draw,inner ysep=18pt]
